Study of SIC and RLS Channel Estimation for Large-Scale Antenna Systems with 1-Bit ADCs

We propose a novel low-resolution-aware recursive least squares channel estimation algorithm for uplink multi-user multiple-input multiple-output systems. In order to reduce the energy consumption, 1-bit ADCs are used on each receive antenna. The loss of performance can be recovered by the large-scale antenna arrays at the receiver. The proposed adaptive channel estimator can mitigate the distortions due to the coarse quantization. Moreover, we propose a low-resolution-aware minimum mean square error based successive interference canceler to successively mitigate the multiuser interference. Simulation results show good performance of the system in terms of mean square error and bit error rate.

==> fig1.tex <==
\pgfplotsset{every axis label/.append style={font=\footnotesize},
	every tick label/.append style={font=\footnotesize},
}

\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor2}{rgb}{0.50000,0.00000,0.50000}%

\begin{tikzpicture}
%[spy using outlines={black,rectangle,magnification=1.5,size=1.5cm, connect spies}]

\begin{axis}[%
width=.8\columnwidth,
height=.6\columnwidth,
at={(0.758in,0.603in)},
scale only axis,
xmin=-20,
xmax=20,
xlabel style={font=\footnotesize},
xlabel={SNR (dB)},
xtick=data,
xmajorgrids,
ymin=-10,
ymax=0,
yminorticks=true,
ylabel style={font=\footnotesize},
ylabel={Normalized MSE (dB)},
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
legend style={at={(0.01,0.01)},anchor=south west,legend cell align=left,align=left,draw=white!15!black,font=\scriptsize}
]

\addplot [color=black,solid,line width=1.0pt,mark=o,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	-20	-0.0675689709722830\\
	-15	-0.144179359129052\\
	-10	-0.333275403268069\\
	-5	-0.980973948735691\\
	0	-1.88985354700679\\
	5	-2.63680971878834\\
	10	-3.07904463524360\\
	15	-3.13098177656343\\
	20	-3.31518076325422\\
};
\addlegendentry{Standard RLS};

\addplot [color=blue,solid,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	-20	-0.176949801689082\\
	-15	-0.464845867249788\\
	-10	-0.948900651230356\\
	-5	-1.72254929607733\\
	0	-2.61610273997104\\
	5	-3.43932955323864\\
	10	-3.88949956875645\\
	15	-3.92860517113319\\
	20	-4.04695112297472\\
};
\addlegendentry{LS \cite{risi}};

\addplot [color=mycolor1,solid,line width=1.0pt,mark=square,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	-20	-0.182946616671307\\
	-15	-0.557890407480466\\
	-10	-1.42660145436821\\
	-5	-3.31013995533732\\
	0	-5.48801014300146\\
	5	-7.20694424547365\\
	10	-8.00444317148157\\
	15	-8.43595488954390\\
	20	-8.48702366258621\\
};
\addlegendentry{LRA-RLS};

\addplot [color=red,solid,line width=1.0pt,mark=triangle,mark options={solid},mark size=3pt]
  table[row sep=crcr]{%
  	-20	-0.187276503642793\\
  	-15	-0.558924997152117\\
  	-10	-1.46420345628233\\
  	-5	-3.39605277807247\\
  	0	-5.85102930118200\\
  	5	-7.80509177683294\\
  	10	-8.66257399541045\\
  	15	-8.89753828816726\\
  	20	-9.18881221521633\\
};
\addlegendentry{BLMMSE \cite{Li}};

\end{axis}

%\spy [blue] on (7.6,4.1) in node [below] at (8.2,3.6);
\end{tikzpicture}%

==> fig2.tex <==
\pgfplotsset{every axis label/.append style={font=\footnotesize},
	every tick label/.append style={font=\footnotesize},
}

\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor2}{rgb}{0.20000,0.80000,0.0000}%

\begin{tikzpicture}

\begin{axis}[%
width=.8\columnwidth,
height=.6\columnwidth,
at={(0.758in,0.603in)},
scale only axis,
xmin=0,
xmax=25,
xlabel style={font=\footnotesize},
xlabel={SNR (dB)},
xtick=data,
xmajorgrids,
ymode=log,
ymin=1e-3,
ymax=0.2,
yminorticks=true,
ylabel style={font=\footnotesize},
ylabel={Uncoded BER},
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
legend style={at={(0.01,0.01)},anchor=south west,legend cell align=left,align=left,draw=white!15!black,font=\scriptsize}
]

\addplot [color=mycolor1,solid,line width=1.0pt,mark=pentagon,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.111250000000000\\
	5	0.0707825000000000\\
	10	0.0547900000000000\\
	15  0.0509975000000000\\
	20	0.0505225000000000\\
	25	0.0493825000000000\\
};
\addlegendentry{MRC \cite{risi}};

\addplot [color=black,solid,line width=1.0pt,mark=+,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0942125000000001\\
	5	0.0371125000000000\\
	10	0.0182600000000000\\
	15  0.0127650000000000\\
	20	0.0108850000000000\\
	25	0.0104175000000000\\
};
\addlegendentry{ZF \cite{risi}};

\addplot [color=mycolor2,solid,line width=1.0pt,mark=square,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0853875000000000\\
	5	0.0336750000000000\\
	10	0.0166000000000000\\
	15  0.0125850000000000\\
	20	0.0113725000000000\\
	25	0.0110450000000000\\
};
\addlegendentry{Traditional MMSE};

\addplot [color=red,solid,line width=1.0pt,mark=triangle,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0835200000000000\\
	5	0.0304525000000000\\
	10	0.0134800000000000\\
	15  0.00967000000000000\\
	20	0.00772250000000000\\
	25	0.00739750000000000\\
};
\addlegendentry{LRA-MMSE};

\addplot [color=blue,solid,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0822275000000000\\
	5	0.0264725000000000\\
	10	0.0107375000000000\\
	15  0.00630500000000000\\
	20	0.00541750000000000\\
	25	0.00529250000000000\\
};
\addlegendentry{LRA-MMSE-SIC};

\end{axis}
\end{tikzpicture}%

==> fig3.tex <==
\pgfplotsset{every axis label/.append style={font=\footnotesize},
	every tick label/.append style={font=\footnotesize},
}

\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor2}{rgb}{0.20000,0.80000,0.0000}%

\begin{tikzpicture}

\begin{axis}[%
width=.8\columnwidth,
height=.6\columnwidth,
at={(0.758in,0.603in)},
scale only axis,
xmin=0,
xmax=25,
xlabel style={font=\footnotesize},
xlabel={$E_b/N_0$ (dB)},
xtick=data,
xmajorgrids,
ymode=log,
ymin=1e-5,
ymax=0.2,
yminorticks=true,
ylabel style={font=\footnotesize},
ylabel={Coded BER},
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
legend entries={ZF \cite{risi},
	Traditional MMSE,
	LRA-MMSE,
LRA-MMSE-SIC},
legend style={at={(0.01,0.01)},anchor=south west,legend cell align=left,align=left,draw=white!15!black,font=\scriptsize}
]

\addlegendimage{color=black,mark=+,line width=1.0pt,mark size=3pt}
\addlegendimage{color=mycolor2,mark=square,line width=1.0pt,mark size=3pt}
\addlegendimage{color=red,mark=triangle,line width=1.0pt,mark size=3pt}
\addlegendimage{color=blue,mark=diamond,line width=1.0pt,mark size=3pt}

\addplot [color=black,solid,line width=1.0pt,mark=+,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.114916666666667\\
	5	0.0333849093614719\\
	10	0.0113115634137427\\
	15  0.00717754871673004\\
	20	0.00585686924131094\\
	25	0.00554782689190700\\
};
%\addlegendentry{ZF \cite{risi}}; % done

\addplot [color=mycolor2,solid,line width=1.0pt,mark=square,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.101817057291667\\
	5	0.0369202473958334\\
	10	0.0113658107452210\\
	15  0.00688850454890068\\
	20	0.00588995005002354\\
	25	0.00545732665067397\\
};
%\addlegendentry{Traditional MMSE}; % done

\addplot [color=red,solid,line width=1.0pt,mark=triangle,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.105262044270833\\
	5	0.0155662763804568\\
	10	0.00338146967351151\\
	15  0.00182980184627399\\
	20	0.00142952278716830\\
	25	0.00121186472284843\\
};
%\addlegendentry{LRA-MMSE}; % done

\addplot [color=blue,solid,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0484856770833333\\
	5	0.00236470306513410\\
	10	0.000285519724641187\\
	15  0.000121685553031152\\
	20	8.99366132695898e-05\\
	25	9.25626354015079e-05\\
};
%\addlegendentry{LRA-MMSE-SIC}; % done

\addplot [color=black,dashed,line width=1.0pt,mark=+,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.155927408854167\\
	5	0.0681464843749999\\
	10	0.0295780213515755\\
	15  0.0194967203069752\\
	20	0.0169618718193384\\
	25	0.0156225385948330\\
};
%\addlegendentry{ZF \cite{risi}};

\addplot [color=mycolor2,dashed,line width=1.0pt,mark=square,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.137888997395833\\
	5	0.0669820963541667\\
	10	0.0301126224269588\\
	15  0.0200629658479961\\
	20	0.0169614301132763\\
	25	0.0166986369159611\\
};
%\addlegendentry{Traditional MMSE}; % done

\addplot [color=red,dashed,line width=1.0pt,mark=triangle,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.155911783854167\\
	5	0.0597568359374999\\
	10	0.0212075160554008\\
	15  0.0130850499532211\\
	20	0.0108665949466127\\
	25	0.00981187264070007\\
};
%\addlegendentry{LRA-MMSE}; % done

\addplot [color=blue,dashed,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.116017903645833\\
	5	0.0222282446172249\\
	10	0.00565078883495146\\
	15  0.00293629807692308\\
	20	0.00232192364066934\\
	25	0.00222564859201640\\
};
%\addlegendentry{LRA-MMSE-SIC}; % done

\addplot[smooth,color=black,solid,line width=1.0pt,mark=none,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
table[row sep=crcr]{%
	1 2\\
};\label{L1}

\addplot[smooth,color=black,dashed,line width=1.0pt,mark=none,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
table[row sep=crcr]{%
	1 2\\
};\label{L2}

\node [draw,fill=white,font=\footnotesize,anchor= north east,at={(24.7,0.17)}] {
	\setlength{\tabcolsep}{0mm}
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{l}
	\ref{L1}{~Perfect CSI}\\
	\ref{L2}{~Estimated CSI}\\
	\end{tabular}
};

\end{axis}
\end{tikzpicture}%

==> fig4.tex <==
\pgfplotsset{every axis label/.append style={font=\footnotesize},
	every tick label/.append style={font=\footnotesize},
}

\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor2}{rgb}{0.50000,0.00000,0.50000}%
\definecolor{mycolor3}{rgb}{0.20000,0.80000,0.0000}%

\begin{tikzpicture}

\begin{axis}[%
width=.8\columnwidth,
height=.6\columnwidth,
at={(0.758in,0.603in)},
scale only axis,
xmin=0,
xmax=25,
xlabel style={font=\footnotesize},
xlabel={$E_b/N_0$ (dB)},
xtick=data,
xmajorgrids,
ymode=log,
ymin=1e-6,
ymax=1,
yminorticks=true,
ylabel style={font=\footnotesize},
ylabel={Coded BER},
ymajorgrids,
yminorgrids,
axis background/.style={fill=white},
legend entries={One terminal w/ 4dB higher transmit energy,
	One terminal w/ 3dB higher transmit energy,
	One terminal w/ 2dB higher transmit energy,
	One terminal w/ 0dB higher transmit energy},
legend style={at={(0.015,0.01)},anchor=south west,legend cell align=left,align=left,draw=white!15!black,font=\scriptsize}
]

\addlegendimage{color=mycolor1,mark=o,line width=1.0pt,mark size=3pt}
\addlegendimage{color=mycolor3,mark=diamond,line width=1.0pt,mark size=3pt}
\addlegendimage{color=mycolor2,mark=square,line width=1.0pt,mark size=3pt}
\addlegendimage{color=blue,mark=triangle,line width=1.0pt,mark size=3pt}

%\addplot [color=black,solid,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
%table[row sep=crcr]{%
%	0	0.262503255208333\\
%	5	0.252643229166667\\
%	10	0.250185546875000\\
%	15  0.247307942708333\\
%	20	0.253727213541667\\
%	25	0.249804687500000\\
%};
%\addlegendentry{Strong interference: 10dB};

%\addplot [color=mycolor1,solid,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
%table[row sep=crcr]{%
%	0	0.113818359375000\\
%	5	0.0484700520833333\\
%	10	0.0281821196933962\\
%	15  0.0257756159855769\\
%	20	0.0236309699292453\\
%	25	0.0235360521788991\\
%};
%\addlegendentry{Strong interference: 5dB};

\addplot [color=mycolor1,solid,line width=1.0pt,mark=o,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0917513020833333\\
	5	0.0228503455996885\\
	10	0.0102664262820513\\
	15  0.00758999208860759\\
	20	0.00596316425120773\\
	25	0.00591240101809955\\
};
%\addlegendentry{Strong interference: 4dB};

\addplot [color=mycolor3,solid,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0727083333333333\\
	5	0.00964522688356164\\
	10	0.00280009143155695\\
	15  0.00188895961934156\\
	20	0.00166015625000000\\
	25	0.00138982771769274\\
};
%\addlegendentry{Strong interference: 3dB};

\addplot [color=mycolor2,solid,line width=1.0pt,mark=square,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0567838541666667\\
	5	0.00606496710526316\\
	10	0.00123200593171296\\
	15  0.000622721354166667\\
	20	0.000420390625000000\\
	25	0.000480143229166667\\
};
%\addlegendentry{Strong interference: 2dB};

\addplot [color=blue,solid,line width=1.0pt,mark=triangle,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.0484856770833333\\
	5	0.00236470306513410\\
	10	0.000285519724641187\\
	15  0.000121685553031152\\
	20	8.99366132695898e-05\\
	25	9.25626354015079e-05\\
};
%\addlegendentry{Strong interference: 0dB};

\addplot [color=mycolor1,dashed,line width=1.0pt,mark=o,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.138629557291667\\
	5	0.0607617187500000\\
	10	0.0309025691105769\\
	15  0.0246738531650641\\
	20	0.0204617210545723\\
	25	0.0196970244984568\\
};
%\addlegendentry{Strong interference: 4dB}; % estimated

\addplot [color=mycolor3,dashed,line width=1.0pt,mark=diamond,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.126337890625000\\
	5	0.0418424479166667\\
	10	0.0184269129672897\\
	15  0.0132807249663978\\
	20	0.0109722548558897\\
	25	0.00885687934027778\\
};
%\addlegendentry{Strong interference: 3dB}; % estimated

\addplot [color=mycolor2,dashed,line width=1.0pt,mark=square,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.118082682291667\\
	5	0.0305468750000000\\
	10	0.0101653454350490\\
	15  0.00722847732843138\\
	20	0.00607518991712707\\
	25	0.00535727446933962\\
};
%\addlegendentry{Strong interference: 2dB}; % estimated

\addplot [color=blue,dashed,line width=1.0pt,mark=triangle,mark options={solid},mark size=3pt]
table[row sep=crcr]{%
	0	0.116017903645833\\
	5	0.0222282446172249\\
	10	0.00565078883495146\\
	15  0.00293629807692308\\
	20	0.00232192364066934\\
	25	0.00222564859201640\\
};
%\addlegendentry{Strong interference: 0dB}; % estimated

\addplot[smooth,color=black,solid,line width=1.0pt,mark=none,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
table[row sep=crcr]{%
	1 2\\
};\label{L111}

\addplot[smooth,color=black,dashed,line width=1.0pt,mark=none,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
table[row sep=crcr]{%
	1 2\\
};\label{L222}

\node [draw,fill=white,font=\footnotesize,anchor= north east,at={(24.7,0.8)}] {
	\setlength{\tabcolsep}{0mm}
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{l}
	\ref{L111}{~Perfect CSI}\\
	\ref{L222}{~Estimated CSI}\\
	\end{tabular}
};

\end{axis}

\end{tikzpicture}%
